Correlations, Bell Inequality Violation & Quantum Entanglement

It is one of the most remarkable features of quantum physics that measurements on spatially separated systems cannot always be described by a locally causal theory. In such a theory, the outcomes of local measurements are determined in advance solely by some unknown (or hidden) variables and the choice of local measurements. Correlations that are allowed within the framework of a locally causal theory are termed classical. Typically, the fact that quantum mechanics does not always result in classical correlations is revealed by the violation of Bell inequalities, which are constraints that have to be satisfied by any classical correlations. It has been known for a long time that entanglement is necessary to demonstrate nonclassical correlations, and hence a Bell inequality violation. However, since some entangled quantum states are known to admit explicit locally causal models, the exact role of entanglement in Bell inequality violation has remained obscure. This thesis provides both a comprehensive review on these issues as well as a report on new discoveries made to clarify the relationship between entanglement and Bell inequality violation.

==> Contribution.tex <==
\begin{center}
{\bf Statement of Originality}\\
\end{center}
I hereby declare that, except where acknowledged below in the
Statement of Contribution to Jointly-published Work and at
other appropriate places in the thesis, the work presented in
this thesis is original and my own work, and has not been
submitted in whole or part for a degree in any university.
%Contributions made by colleagues at UQ and elsewhere to the
%content of this thesis and related joint-published work is
%fully acknowledged at appropriate places in the thesis.\\

\begin{center}
{\bf Statement of Contribution to Jointly-published Work}\\
\end{center}

The content of Chapter~\ref{Chap:QuantumBounds} is based
largely on Ref.~\cite{Y.C.Liang:PRA:2007}, which results from a
joint research project between me and my supervisor Andrew C.
Doherty. I have done all the research in this chapter guided by
initial ideas of Andrew C. Doherty and weekly discussion about
the project. I wrote the initial draft of
Ref.~\cite{Y.C.Liang:PRA:2007}.\\

The content of Chapter~\ref{Chap:BellViolation} is based
largely on Ref.~\cite{Y.C.Liang:PRA:2006}, which results from a
joint research project between me and my supervisor Andrew C.
Doherty. Except for Sec.~\ref{Sec:I22nnViolation}, which
consists mostly of review material, I have done all the
research in this chapter guided by initial ideas of Andrew C.
Doherty and weekly discussion about the project.
I wrote the initial draft of Ref.~\cite{Y.C.Liang:PRA:2006}.\\

The content of Sec.~\ref{Sec:Nonlocality:All} and
Appendix~\ref{App:SLOCC} are based largely on
Ref.~\cite{Ll.Masanes:0703268} and
Ref.~\cite{Y.C.Liang:0710.5350}, which result from a joint
research project between me and my collaborators Llu\'{\i}s
Masanes and Andrew C. Doherty. Ref.~\cite{Ll.Masanes:0703268}
and Ref.~\cite{Y.C.Liang:0710.5350} were initially drafted,
respectively, by Llu\'{\i}s Masanes and me. This project was
initiated by Llu\'{\i}s Masanes who also did many of the
initial calculations. The present form of Lemma 1 and Lemma 2
in Ref.~\cite{Ll.Masanes:0703268} is a result of collaborations
between the three of us. Results presented in Sec. II of
Ref.~\cite{Y.C.Liang:0710.5350} were obtained by Llu\'{\i}s
Masanes and me, guided by weekly discussion with Andrew C.
Doherty.  Results presented in Sec. III C of
Ref.~\cite{Y.C.Liang:0710.5350} was initially obtained by
Llu\'{\i}s Masanes and independently verified by me. Results
presented in Sec. IV of Ref.~\cite{Y.C.Liang:0710.5350} were
initially obtained by me and independently verified by
Llu\'{\i}s Masanes.\\



%----------------------------------------------------------------



%\documentclass[a4paper,12pt]{article}
%\usepackage{amsmath,graphicx,epsfig,color,hyperref}
%
%%\setlength{\textwidth}{19.5cm} \setlength{\textheight}{25.5cm}
%%\setlength{\parindent}{20pt} \setlength{\oddsidemargin}{-1.8cm}
%%\setlength{\topmargin}{-2cm}
%
%\begin{document}
%
%\begin{center}
%{\bf Statement of Originality}\\
%\end{center}
%I hereby declare that, except where acknowledged below in the
%Statement of Contribution to Jointly-published Work and at
%other appropriate places in the thesis, the work presented in
%this thesis is original and my own work, and has not been
%submitted in whole or part for a degree in any university.
%%Contributions made by colleagues at UQ and elsewhere to the
%%content of this thesis and related joint-published work is
%%fully acknowledged at appropriate places in the thesis.\\
%
%\begin{center}
%{\bf Statement of Contribution to Jointly-published Work}\\
%\end{center}
%
%The content of Chapter~\ref{Chap:QuantumBounds} is based
%largely on Ref.~\cite{Y.C.Liang:PRA:2007}, which results from a
%joint research project between me and my supervisor Andrew C.
%Doherty. I have done all the research in this chapter guided by
%initial ideas of Andrew C. Doherty and weekly discussion about
%the project. Ref.~\cite{Y.C.Liang:PRA:2007} was initially
%drafted by me.\\
%
%The content of Chapter~\ref{Chap:BellViolation} is based
%largely on Ref.~\cite{Y.C.Liang:PRA:2006}, which results from a
%joint research project between me and my supervisor Andrew C.
%Doherty. Except for Sec.~\ref{Sec:I22nnViolation}, which
%consists mostly of review material, I have done all the
%research in this chapter guided by initial ideas of Andrew C.
%Doherty and weekly discussion about the project.
%Ref.~\cite{Y.C.Liang:PRA:2006} was initially drafted by me.\\
%
%The content of Sec.~\ref{Sec:Nonlocality:All} and
%Appendix~\ref{App:SLOCC} are based largely on
%Ref.~\cite{Ll.Masanes:0703268} and
%Ref.~\cite{Y.C.Liang:0710.5350}, which result from a joint
%research project between me and my collaborators Llu\'{\i}s
%Masanes and Andrew C. Doherty. Ref.~\cite{Ll.Masanes:0703268}
%and Ref.~\cite{Y.C.Liang:0710.5350} were initially drafted,
%respectively, by Llu\'{\i}s Masanes and me. This project was
%initiated by Llu\'{\i}s Masanes who also did many of the
%initial calculations. The present form of Lemma 1 and Lemma 2
%in Ref.~\cite{Ll.Masanes:0703268} is a result of collaborations
%between all the three of us. Results presented in Sec. II of
%Ref.~\cite{Y.C.Liang:0710.5350} were obtained by Llu\'{\i}s
%Masanes and me, who was guided by weekly discussion with Andrew
%C. Doherty.  Results presented in Sec. III C of
%Ref.~\cite{Y.C.Liang:0710.5350} was initially obtained by
%Llu\'{\i}s Masanes and independently verified by me. Results
%presented in Sec. IV of Ref.~\cite{Y.C.Liang:0710.5350} was
%initially obtained by me and independently verified by
%Llu\'{\i}s Masanes.\\
%
%
%%\bibliography{Bell.Entanglement.Nonlocality}
%
%
%\end{document}


==> dedication.tex <==
\vphantom{d}
\vspace{5cm}
\begin{center}
{\em
    {\large To my beloved family members in Malaysia}\\
    \vspace{0.5cm}
    {\large and my dearest Shih-yin,}\\
    \vspace{0.5cm}
    {\large for their continuous support, encouragement and love $\ldots$}
}
\end{center}
\vfill


==> quotation.tex <==
\begin{quote}
``{\em For those who are not shocked when they first come across
quantum theory cannot possibly have understood it}", Niels Bohr,
first quoted by Werner Heisenberg in Physics and Beyond, pp.~206 (New
York: Harper \& Row, 1971).
\end{quote}

\vspace{0.5cm}
\begin{quote}
``{\em When the `system' in question is the whole world where
is the `measurer' to be found? Inside, rather than outside,
presumably. What exactly qualifies some subsystems to play this
role? Was the world wave function waiting to jump for thousands
of millions of years until a single-celled living creature
appeared? Or did it have to wait a little longer for some
highly qualified measurer --- with a Ph.D.?}\,", John S.~Bell
in Quantum Gravity 2, pp. 611 (1981).
\end{quote}

\vspace{0.5cm}
\begin{quote}
``{\em $\ldots$ we have always had a great deal of difficulty
understanding the world view that quantum mechanics represents.
At least I do, because I'm an old enough man that I haven't got
to the point that this stuff is obvious to me. Okay, I still
get nervous with it $\ldots$ you know how it always is, every
new idea, it takes a generation or two until it becomes obvious
that there's no real problem. I cannot define the real problem,
therefore I suspect there's no real problem, but I'm not sure
there's no real problem}", Richard~P.~Feynman in International
Journal of Theoretical Physics, {\bf 21}, pp.~467 (1982).
\end{quote}

\vspace{0.5cm}
\begin{quote}
``{\em We often discussed his notions on objective reality. I recall
that during one walk Einstein suddenly stopped, turned to me and
asked whether I really believed that the moon exists only when I look
at it. The rest of this walk was devoted to a discussion of what a
physicist should mean by the term `to exist'~}", A.~Pais, Reviews of
Modern Physics, {\bf 51}, pp.~908 (1979).
\end{quote}

\vspace{0.5cm}
\begin{quote}
``{\em Bell's theorem is the most profound discovery of science}",
Henry P. Stapp, IL Nuovo Cimento, {\bf 29B}, pp.~271 (1975).
\end{quote}

\vspace{0.5cm}
\begin{quote}
``{\em Anybody who's not bothered by Bell's theorem has to have
rocks in his head}", anonymous Princeton physicist, first
quoted by N.~David Mermin in Physics Today, {\bf 38}, pp.~41
(1985).
\end{quote}

